Efficient p-multigrid spectral element model for water waves and marine offshore structures

In marine offshore engineering, cost-efficient simulation of unsteady water waves and their nonlinear interaction with bodies are important to address a broad range of engineering applications at increasing fidelity and scale. We consider a fully nonlinear potential flow (FNPF) model discretized using a Galerkin spectral element method to serve as a basis for handling both wave propagation and wave-body interaction with high computational efficiency within a single modellingapproach. We design and propose an efficientO(n)-scalable computational procedure based on geometric p-multigrid for solving the Laplace problem in the numerical scheme. The fluid volume and the geometric features of complex bodies is represented accurately using high-order polynomial basis functions and unstructured meshes with curvilinear prism elements. The new p-multigrid spectralelement model can take advantage of the high-order polynomial basis and thereby avoid generating a hierarchy of geometric meshes with changing number of elements as required in geometric h-multigrid approaches. We provide numerical benchmarks for the algorithmic and numerical efficiency of the iterative geometric p-multigrid solver. Results of numerical experiments are presented for wave propagation and for wave-body interaction in an advanced case for focusing design waves interacting with a FPSO. Our study shows, that the use of iterative geometric p-multigrid methods for theLaplace problem can significantly improve run-time efficiency of FNPF simulators.

==> ditched.tex <==
\subsubsection{Condensed system results}

Another approach is to apply a MG solver on the condensed system eq. \eqref{eq:u_B_cond}. It decreases computational time for the MG solver by a large margin as the linear system of equations is better conditioned with less degrees of freedom. An efficient way of factorizing the inner nodes matrix $L_{ii}$ is described in \cite{HUISMANN2017437}. 

[TBD: explanation and maybe example of scaling?]

A strength of applying SC is that there is no need of storing smoothing matrix as the cost of assembly this matrix will be now much lower than in the full system.

Table \ref{table:BarTest_iterc} depicts average iteration number and \ref{table:BarTest_WUc} time (in WUs) to achieve a given tolerance.

\FloatBarrier
\begin{table}[!htbp]
\centering
\caption{Average number of iterations to achieve given tolerance. Full system.}
\label{table:BarTest_iterc}
\begin{tabular}{@{}lcccc@{}} \toprule
Method & $tol=1e-4$ & $tol=1e-5$ & $tol=1e-6$ & $tol=1e-7$ \\ \midrule
%\multicolumn{8}{c}
MGCG(3,3) I & 1.00 & 1.97 & 1.99 & 1.99 \\
MGCG(3,3) II & 1.00 & 1.97 & 1.99 & 1.99 \\
MGCG(3,3) III & 1.00 & 1.97 & 1.99 & 1.99 \\
MG(3,3) I & 1.00 & 1.97 & 1.99 & 1.99 \\
MGDC(3,3) I & 1.00 & 1.97 & 1.99 & 1.99 \\
\bottomrule
\end{tabular}
\end{table}
\FloatBarrier

\FloatBarrier
\begin{table}[!htbp]
\centering
\caption{Average cost to achieve given tolerance in the absolute WUs (relative to the size of the full system) for full systems.}
\label{table:BarTest_WUc}
\begin{tabular}{@{}lcccc@{}} \toprule
Method & $tol=1e-4$ & $tol=1e-5$ & $tol=1e-6$ & $tol=1e-7$ \\ \midrule
% \multicolumn{8}{c}
MGCG(3,3) I & 2.37 & 4.65 & 4.62 & 4.87 \\
MGCG(3,3) II & 2.39 & 4.60 & 4.68 & 4.77 \\
MGCG(3,3) III & 2.35 & 4.79 & 4.68 & 4.71 \\
MG(3,3) I & 2.65 & 4.68 & 4.93 & 4.63 \\
MGDC(3,3) I & 2.75 & 4.56 & 4.63 & 4.77 \\
\bottomrule
\end{tabular}
\end{table}
\FloatBarrier

\subsection{Static Condensation}

We use $p$-multigrid to solve the sparse linear system  \eqref{eq:laplaceproblemdiscrete} directly, and also a statically condensed system \cite{star_and_cond,cond_huis}, where the coefficient matrix is then the Schur complement of the coefficient matrix $\mathcal{L}$. The coefficient matrix and the right hand side vector are decomposed according to 

\begin{equation}
\label{eq:Aub_cond}
\begin{pmatrix} 
A_{bb} & A_{bi} \\
A_{ib} & A_{ii} 
\end{pmatrix}
\quad
\begin{pmatrix} 
\phi_{b} \\
\phi_{b} 
\end{pmatrix}
\quad = \quad 
\begin{pmatrix} 
b_{b} \\
b_{i}.
\end{pmatrix},
\end{equation}


\begin{align}
    \mathcal{L}=\left[ \begin{array}{cc} \mathcal{L}_{bb} & \mathcal{L}_{bi} \\ \mathcal{L}_{ib} & \mathcal{L}_{ii} \end{array} \right], \quad {\bf b}=\left[ \begin{array}{c} {\bf b}_{b } \\ {\bf b}_{i} \end{array} \right],
\end{align}
resulting in the condensed system
%
\begin{align}
(\mathcal{L}_{bb} - \mathcal{L}_{bi} \mathcal{L}_{ii}^{-1} \mathcal{L}_{ib}) \phi_b = {\bf b}_b - \mathcal{L}_{bi} \mathcal{L}_{ii}^{-1} {\bf b}_i.
\label{eq:laplacecondensed}
\end{align}
%
which can be obtained using \emph{Static Condensation}. Static Condensation is a variant of the non-overlapping Schur complement method. Following  one can split \eqref{eq:Auf} into 
%

%
where the subscripts \textit{B} denotes nodes on the element's edge and \textit{I} interior elements (see figure \ref{fig:cond}). Then, boundary values $u_B$ can be solved from the equation $(A_{BB} - A_{BI} {(A_{II})}^{-1} A_{IB}) u_B = f_B - A_{BI} {(A_{II})}^{-1} f_I$ and the interior nodes, based on the edge nodes $u_B$: $A_{II} u_I = (f_I - A_{IB} u_B)$.












\begin{figure}[H]
\subfloat[ \label{subfig:el_smoother}]{%
  \includegraphics[width=0.45\textwidth]{figures/inkdrawings/elementbased_relaxation.eps}
}
\hfill
\subfloat[\label{subfig:star_smoother}]{%
  \includegraphics[width=0.45\textwidth]{figures/inkdrawings/star_relaxation.eps}
}
\caption{Overlapping regions with Dirichlet boundary conditions treatment at the north edges. On the left: element-centered block smoother with 2 overlapping nodes to the east and west. On the right: vertex-center ("star") block smoother with a whole edge of overlapping region in all spatial directions.}
\label{fig:smoothing}
\end{figure}


% The prolongation operator $\mathcal{P}_c^f$ is defined in terms of a Lagrange polynomial $h_j^c({\bf x})$ that is defined in terms of the node distribution of the coarse mesh elements. For $\forall i \in \{ 0,...,N_f \}$, $\forall j \in \{ 0,...,N_c \}$

\FloatBarrier
\begin{table}[!htbp]
\centering
\caption{Coarsening strategy.}
\label{table:BTcoarse3D2}
\begin{tabular}{@{}lccc@{}} \toprule
Grid level & 3 & 2 & 1 \\ \midrule
% \multicolumn{8}{c}
 $P_{xy}$ & 5 & 3 & 1  \\
 $P_z$ & 3 & 3 & 1 \\
 \bottomrule
\end{tabular}
\end{table}
\FloatBarrier
